Detecting Flow Gaps in Data Streams

Data stream monitoring is a crucial task which has a wide range of applications. The majority of existing research in this area can be broadly classified into two types, monitoring value sum and monitoring value cardinality. In this paper, we define a third type, monitoring value variation, which can help us detect flow gaps in data streams. To realize this function, we propose GapFilter, leveraging the idea of Sketch for achieving speed and accuracy. To the best of our knowledge, this is the first work to detect flow gaps in data streams. Two key ideas of our work are the similarity absorption technique and the civilian-suspect mechanism. The similarity absorption technique helps in reducing memory usage and enhancing speed, while the civilian-suspect mechanism further boosts accuracy by organically integrating broad monitoring of overall flows with meticulous monitoring of suspicious flows.We have developed two versions of GapFilter. Speed-Oriented GapFilter (GapFilter-SO) emphasizes speed while maintaining satisfactory accuracy. Accuracy-Oriented GapFilter (GapFilter-AO) prioritizes accuracy while ensuring considerable speed. We provide a theoretical proof demonstrating that GapFilter secures high accuracy with minimal memory usage. Further, extensive experiments were conducted to assess the accuracy and speed of our algorithms. The results reveal that GapFilter-AO requires, on average, 1/32 of the memory to match the accuracy of the Straw-man solution. GapFilter-SO operates at a speed 3 times faster than the Straw-man solution. All associated source code has been open-sourced and is available on GitHub.

==> SIGMOD21/zyk/exp_veri.tex <==

To verify the correctness of Lemma~\ref{lem:error} and Theorem~\ref{theo:freezing_bound}, we show two kinds of variance bound.
%
Lemma~\ref{lem:error} provides a $\mathcal{P}$-independent loss bound, and an $\mathcal{R}$-dependent tight bound.
%
We use SpaceSaving and Randomized Admission Policy as the strategy $\mathcal{P}$, and vary the length $w$ of the count part.
%
%
As shown in Figure~\ref{fig:bound}, we plot the loose upper bounds, the tight upper bounds, 
%
and the sample variances of the hot panning version and the early freezing version.
%
%
It can be found that the bounds of variances are always greater than the sample variances of the hot panning version,
%
and then greater than the sample variances of the early freezing version, which verifies our theorems and shows the benefits of Early Freezing.
%
%
It is worth noting two points:
%
1) The tight bounds are extremely close to the sample variances, which indicates our bounds are accurate.
%
2) Panning hot items to reduce the redundancy is beneficial to reduce variance, 
%
and the strategy of finding top-$K$ frequent items more accurately has a smaller variance.


